Optimal Link Adaptation for Multicarrier Communication Systems

Link adaptation is the terminology used to describe techniques that improve multicarrier communication systems performance by dynamically adapting the transmission parameters, i.e., transmit power and number of bits per subcarrier, to the changing quality of the wireless link. The research literature has focused on single objective optimization techniques to optimize the multicarrier communication systems performance, e.g., maximizing the throughput/capacity or minimizing the transmit power subject to a set of constraints. In this dissertation, we adopt a novel optimization concept, namely multiobjective optimization, where our objective is to simultaneously optimize the conflicting and incommensurable throughput and power objectives. More specifically, in some of the following Chapters, we propose novel algorithms that jointly maximize the multicarrier system throughput and minimize its total transmit power subject to quality-of-service, total transmit power, and maximum allocated bits per subcarrier constraints. The proposed algorithms require prior knowledge about the importance of the competing objective functions in terms of pre-determined weighting coefficients, or they can adapt the weighting coefficients during the solution process while meeting the constraints, in order to reduce the computational complexity. Simulation results show significant performance gains in terms of the achieved throughput and transmit power when compared to single optimization approaches, at the cost of no additional complexity.

==> Ch_2/Ch_2_Conflict_.tex <==
\chapter{Joint Optimization of Bit and Power Loading for Multicarrier Systems} \label{ch:WCL}
\input{Ch_2/abstract}
\input{Ch_2/intro}
\input{Ch_2/opt}
\input{Ch_2/sim}
\input{Ch_2/conclusion}
\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,C:/Users/ebedeer/Sync/Google_Drive/z_Work/Research/Project_CRC/Written_Material/Publications/mybib_file}
%\bibliography{IEEEabrv,D:/Ebrahim/Sync/Google_Drive/z_Work/Research/Project_CRC/Written_Material/Publications/mybib_file} 

==> authorship/author.tex <==
\chapter*{Co-Authorship Statement}

I, Ebrahim E. Bedeer-Mohamed, hold a principle author status for all the manuscript chapters (Chapter 2 - 6) in this dissertation. However, each manuscript is co-authored by my supervisors and co-researchers, whose contributions have facilitated the development of this work as described below.

\begin{itemize}
	\item Paper 1 in Chapter \ref{ch:TVT_GA}:
	Ebrahim Bedeer, Octavia Dobre, Mohamed H. Ahmed, and Kareem Baddour, ``A Novel Multiobjective Optimization Approach to Bit and Power Allocation for OFDM Systems,'' under review, IEEE Transactions on Mobile Computing. \\
	I was the primary author and with authors 2 - 4 contributed to the idea, its formulation and development, and refinement of the presentation.
	\item Paper 2 in Chapter \ref{ch:WCL}:
	Ebrahim Bedeer, Octavia Dobre, Mohamed H. Ahmed, and Kareem Baddour, ``Joint Optimization of Bit and Power Loading for Multicarrier Systems,'' IEEE Wireless Communications Letters, vol. 2, no. 4, pp. 447-450, Aug. 2013. \\	
	I was the primary author and with authors 2 - 4 contributed to the idea, its formulation and development, and refinement of the presentation.
	\item Paper 3 in Chapter \ref{ch:TW}:
	Ebrahim Bedeer, Octavia Dobre, Mohamed H. Ahmed, and Kareem Baddour, ``A Multiobjective Optimization Approach for Optimal Link Adaptation of OFDM-based Cognitive Radio Systems with Imperfect Spectrum Sensing,'' IEEE Transactions on Wireless Communications, vol. 13, no. 4, pp. 2339-2351, Apr. 2014. \\
	I was the primary author and with authors 2 - 4 contributed to the idea, its formulation and development, and refinement of the presentation.	
	\item Paper 4 in Chapter \ref{ch:TVT_MOOP}:
	Ebrahim Bedeer, Octavia Dobre, Mohamed H. Ahmed, and Kareem Baddour, ``Rate-Interference Tradeoff in OFDM-based Cognitive Radio Systems,'' major revisions, IEEE Transactions on vehicular Technology. \\
	I was the primary author and with authors 2 - 4 contributed to the idea, its formulation and development, and refinement of the presentation.	
	\item Paper 5 in Chapter \ref{ch:TVT_EE}:
	Ebrahim Bedeer, Osama Amin, Octavia Dobre, Mohamed H. Ahmed, and Kareem Baddour, ``Energy-Efficient Power Loading for OFDM-based Cognitive Radio Systems with Channel Uncertainties,'' accepted with minor revisions, IEEE Transactions on vehicular Technology.	\\
	I was the primary author and with authors 2 - 5 contributed to the idea, its formulation and development, and refinement of the presentation.	
\end{itemize}




\doubleSignature{}{Ebrahim E. Bedeer-Mohamed}{Date}
%\Signature{}{\hspace{40pt}Ebrahim E. Bedeer-Mohamed \hspace{5cm} Date}
%\Signature{G\"ottingen}{David Hilbert}{Emmy Noether}{Hermann Minkowski} 

==> losymbols.tex <==
% The following definitions will go in the main glossary

%\newglossaryentry{culdesac}{name=cul-de-sac,description={passage
%or street closed at one end},plural=culs-de-sac}
%
%\newglossaryentry{elite}{name={\'e}lite,description={select
%group or class},sort=elite}
%
%\newglossaryentry{elitism}{name={\'e}litism,description={advocacy
%of dominance by an \gls{elite}},sort=elitism}
%
%\newglossaryentry{attache}{name=attach\'e,
%description={person with special diplomatic responsibilities}}

% The following definitions will go in the list of acronyms

\newacronym{1}{$\mathbf{X}$}{Bold-faced upper case letters to denote matrices}
\newacronym{2}{$\mathbf{x}$}{Bold-faced lower case letters for vectors}
\newacronym{3}{$x$}{Light-faced letters for scalar quantities}
\newacronym{4}{$\mathbf{I}$}{Identity matrix}
\newacronym{5}{$[.]^T$}{Transpose operation}
\newacronym{6}{$\nabla$}{Gradient Operator}
\newacronym{7}{$\lfloor x \rfloor$}{Largest integer not greater than $x$}
\newacronym{8}{$x^*$}{Optimal value of $x$}
\newacronym{9}{$\mathcal{OP}$}{Optimization Problem}
\newacronym{10}{$\lfloor x \rceil$}{Nearest integer to $x$}
\newacronym{11}{$[x,y]^-$}{$\min(x,y)$}
\newacronym{12}{$[x]^+$}{$\max(0,x)$}
\newacronym{13}{$\mathbb{X}$}{Set}
\newacronym{14}{$\bar{\bar{\mathbb{X}}}$}{Cardinality of the set $\mathbb{X}$}
\newacronym{15}{$\mathcal{O}(.)$}{Big-oh notation}
\newacronym{16}{$\exp(.)$}{The exponential function}
\newacronym{17}{$\log(.)$}{The logarithmic function to the base of 10}
\newacronym{18}{$\ln(.)$}{The natural logarithmic function}
\newacronym{19}{$\log_2(.)$}{The logarithmic function to the base of 2}
\newacronym{20}{$f(.)$}{Objective function}
\newacronym{21}{$g(.)$}{Inequality constraints}
\newacronym{22}{$\mathbf{f}(.)$}{Objective functions vector}
\newacronym{23}{$\mathcal{G}(.)$}{Equality constraints}
\newacronym{24}{$\mathbb{E}(.)$}{Expectation operator}

%\newacronym{eeprom}{EEPROM}{electrically erasable programmable
%read-only memory}

% The following definitions will go in the list of symbols

%\newglossaryentry{1}{type=symbols,name=$\mathcal{P}_i$,symbol={\ensuremath{\Omega}},description=Power per subcarrier $i$}

%\newglossaryentry{CR}{name={\large{\textbf{MCM system in CR environment parameters: }}},description={\nopostdesc}}
%\newglossaryentry{ch}{name={\large{\textbf{Channel parameters:}}},description={\nopostdesc}}
%\newglossaryentry{LM}{name={\large{\textbf{Levenberg-Marquardt algorithm parameters:}}},description={\nopostdesc}}
%\newglossaryentry{OP}{name={\large{\textbf{Optimization parameters:}}},description={\nopostdesc}}
%\newglossaryentry{MCM}{name={\large{\textbf{MCM system in non-CR environment parameters:}}},description={\nopostdesc}}

\newglossaryentry{s1}{type=symbols,name=$p_i$,description= Power per subcarrier $i$}
\newglossaryentry{s2}{type=symbols,name=$N$,description= Number of subcarriers}
\newglossaryentry{s3}{type=symbols,name=$i$,description= Index of subcarrier}
\newglossaryentry{s4}{type=symbols,name=$b_i$,description= Number of bits per subcarrier $i$}
\newglossaryentry{s5}{type=symbols,name=$C$,description= Number of inequality constraints}
\newglossaryentry{s7}{type=symbols,name=$O$,description= Number of objective functions}
\newglossaryentry{s8}{type=symbols,name=$\textup{BER}_{\rm{av}}$,description= Average BER}
\newglossaryentry{s9}{type=symbols,name=$\textup{BER}_{\rm{th}}$,description= Threshold value of BER}
\newglossaryentry{s10}{type=symbols,name=$\textup{BER}_{i}$,description= BER per subcarrier $i$}
\newglossaryentry{s11}{type=symbols,name=$\mathcal{H}_i$,description= Channel coefficient of subcarrier $i$}
\newglossaryentry{s12}{type=symbols,name=$\sigma^2_n$,description= Variance of the additive white Gaussian noise}
\newglossaryentry{s13}{type=symbols,name=$P_{\rm{th}}$,description= Threshold value on the total transmit power}
\newglossaryentry{s14}{type=symbols,name=$\mathbf{p}$,description= $N$-dimensional power allocation vector}
\newglossaryentry{s15}{type=symbols,name=$\mathbf{b}$,description= $N$-dimensional bit allocation vector}
\newglossaryentry{s16}{type=symbols,name=$\alpha$,description= Weighting parameter}
\newglossaryentry{s17}{type=symbols,name=$\ell$,description= Index of subchannel}
\newglossaryentry{s18}{type=symbols,name=$b_{i,\rm{max}}$,description= Maximum number of bits allocated to subcarrier $i$}
\newglossaryentry{s19}{type=symbols,name=$\gamma_i$,description= Channel-to-noise ratio or channel-to-noise-plus-interference for subcarrier $i$}
\newglossaryentry{s20}{type=symbols,name=$y^2$,description= Non-negative slack variable}
\newglossaryentry{s21}{type=symbols,name=$\xi$,description= Scale parameter of Laplace distribution}
\newglossaryentry{s22}{type=symbols,name=$\textbf{y}$,description= Vector of slack variables}
\newglossaryentry{s23}{type=symbols,name=$\mathcal{L(.)}$,description= Lagrange function}
\newglossaryentry{s24}{type=symbols,name=$\boldsymbol\lambda$,description= Vector of Lagrange multipliers}
\newglossaryentry{s25}{type=symbols,name=$\lambda$,description= Lagrange multiplier}
\newglossaryentry{s26}{type=symbols,name=$u_{\rm{p}}$,description= Normalization factor for the transmit power objective}
\newglossaryentry{s27}{type=symbols,name=$u_{\rm{b}}$,description= Normalization factor for the throughput objective}
\newglossaryentry{s28}{type=symbols,name=$\textup{BER}_{{\rm{th}},i}$,description= Threshold value on the BER per subcarrier $i$}
\newglossaryentry{s29}{type=symbols,name=$\Gamma_i$,description= Signal-to-noise ratio gap per subcarrier $i$}
\newglossaryentry{s30}{type=symbols,name=$\epsilon$,description= Tolerance error}
%\newglossaryentry{s31}{type=symbols,name=$\varepsilon$,description= Tolerance error}
\newglossaryentry{s32}{type=symbols,name=$\gamma_{{\rm{th}},i}^{\rm{max}}$,description= Maximum $\gamma_i$}
\newglossaryentry{s33}{type=symbols,name=$\nu$,description= Inverse of the mean of exponential distribution}
\newglossaryentry{s34}{type=symbols,name=$\gamma_{{\rm{th}},i}^{\rm{min}}$,description= Minimum $\gamma_i$}
\newglossaryentry{s35}{type=symbols,name=$a$,description= Location parameter of Laplace distribution}
\newglossaryentry{s36}{type=symbols,name=$\vartheta_k$,description= Laplace distributed random number}
\newglossaryentry{s37}{type=symbols,name=$r_k$,description= Uniformly distributed random variable}
%\newglossaryentry{s38}{type=symbols,name=$\textbf{y}$,description= Vector of slack variables}
\newglossaryentry{s39}{type=symbols,name=$L$,description= Number of subchannels or PUs}
\newglossaryentry{s40}{type=symbols,name=$m$,description= Index of subchannel}
\newglossaryentry{s41}{type=symbols,name=$B_m$,description= Bandwidth of subchannel of PU $m$}
\newglossaryentry{s42}{type=symbols,name=$\upsilon_k$,description= Uniformly distributed random number}
\newglossaryentry{s43}{type=symbols,name=$\beta_{{\rm{ov}}}^{(m)}$,description= Probability that subchannel $m$ is truly occupied under the condition that the SU identified it to be vacant}
\newglossaryentry{s44}{type=symbols,name=$\rho^{(m)}$,description= Probability that the PU transmits on subchannel $m$}
\newglossaryentry{s45}{type=symbols,name=$w_k$,description= Offspring}
\newglossaryentry{s46}{type=symbols,name=$PL(.)$,description= Path loss}
\newglossaryentry{s47}{type=symbols,name=$d_m$,description= Distance between SU and the PU $m$}
\newglossaryentry{s48}{type=symbols,name=$d_0$,description= Reference distance}
\newglossaryentry{s49}{type=symbols,name=$\mathcal{H}_{{\rm{sp}}}^{(m)}$,description= Channel coeefficient between SU and PU $m$}
\newglossaryentry{s50}{type=symbols,name=$z_k$,description= Parent}
\newglossaryentry{s51}{type=symbols,name=$z^{(l)}$,description= Lower bound on the decision variable}
\newglossaryentry{s52}{type=symbols,name=$T_{s,m}$,description= Symbol duration of the SU $m$}
\newglossaryentry{s53}{type=symbols,name=$d_{\ell}$,description= Distance between SU and PU $\ell$}
\newglossaryentry{s54}{type=symbols,name=$f_{i,\ell}$,description= Spectral distance between subcarrier $i$ of SU $m$ and PU $\ell$ frequency band}
\newglossaryentry{s55}{type=symbols,name=$B_{\ell}$,description= Bandwidth of subchannel or PU $\ell$}
\newglossaryentry{s56}{type=symbols,name=$z^{(u)}$,description= Upper bound on the decision variable}
\newglossaryentry{s57}{type=symbols,name=$\rho^{(m)}_{{\rm{md}}}$,description= Probability of mis-detection at PU $m$}
\newglossaryentry{s58}{type=symbols,name=$\rho^{(\ell)}_{{\rm{fa}}}$,description= Probability of false-alarm at PU $\ell$}
\newglossaryentry{s59}{type=symbols,name=$\beta_{{\rm{oo}}}^{(\ell)} $,description= Probability that subchannel $\ell$ is truly occupied by the PU under the condition that the SU identified it to be occupied}
\newglossaryentry{s60}{type=symbols,name=$P_{\textup{th}}^{(m)}$,description= CCI threshold at PU $m$}
\newglossaryentry{s61}{type=symbols,name=$P_{\textup{th}}^{(\ell)}$,description= ACI threshold at PU $\ell$}
\newglossaryentry{s62}{type=symbols,name=$\Psi_{{\rm{th}}}^{(m)}$,description= Probability to satisfy the CCI constraint at PU $m$}
\newglossaryentry{s63}{type=symbols,name=$\Psi_{{\rm{th}}}^{(\ell)}$,description= Probability to satisfy the ACI constraint at PU $\ell$}
\newglossaryentry{s64}{type=symbols,name=$X^{(m)}$,description= Channel information coefficient at PU $m$}
\newglossaryentry{s65}{type=symbols,name=$X^{(\ell)}$,description= Channel information coefficient at PU $\ell$}
\newglossaryentry{s66}{type=symbols,name=$u_{\rm{CCI}}$,description= Normalization factor for the CCI objective function}
\newglossaryentry{s67}{type=symbols,name=$u_{\rm{ACI}}$,description= Normalization factor for the ACI objective function}
\newglossaryentry{s68}{type=symbols,name=$u_{\rm{rate}}$,description= Normalization factor for the transmission rate objective function}
\newglossaryentry{s69}{type=symbols,name=$\alpha_{\rm{CCI}}$,description= Weighting coefficient for the CCI objective function}
\newglossaryentry{s70}{type=symbols,name=$\alpha_{\rm{ACI}}$,description= Weighting coefficient for the ACI objective function}
\newglossaryentry{s71}{type=symbols,name=$\alpha_{\rm{rate}}$,description= Weighting coefficient for the transmission rate objective function}
\newglossaryentry{s72}{type=symbols,name=$\kappa$,description= Constant that depends on power amplifier efficiency}
\newglossaryentry{s73}{type=symbols,name=$p_{\rm{c}}$,description= Circuit power consumption}
\newglossaryentry{s74}{type=symbols,name=$R_{\rm{th}}$,description= Minimum supported rate}
\newglossaryentry{s75}{type=symbols,name=$\varrho$,description= Index of constraints}
\newglossaryentry{s76}{type=symbols,name=$N_{\rm{ch}}$,description= Order of fading channel}
\newglossaryentry{s77}{type=symbols,name=$\mathbf{h}$,description= Impulse response of fading channel}
\newglossaryentry{s78}{type=symbols,name=$\bf{b}_{\rm{pilot}}$,description= Training pilot symbols}
\newglossaryentry{s79}{type=symbols,name=$\bf{\hat h}$,description= Estimate of impulse response of fading channel}
\newglossaryentry{s80}{type=symbols,name=$\bf{B}$,description= Circulant matrix}
\newglossaryentry{s81}{type=symbols,name=$\bf{F}$,description= Discrete Fourier transform matrix}
\newglossaryentry{s82}{type=symbols,name=$\Delta f$,description= Subcarrier bandwidth}
\newglossaryentry{s83}{type=symbols,name=$\mathcal{J}_i$,description= Interference from the PUs to subcarrier $i$ of the SU}
\newglossaryentry{s84}{type=symbols,name=$\sigma _{\Delta H}^2$,description= Minimum mean squre error of the channel estimate}
\newglossaryentry{s85}{type=symbols,name=$P_{\rm{pilots}}$,description= Pilots' transmit power}
\newglossaryentry{s86}{type=symbols,name=$\eta_{\rm{EE}}$,description= Energy efficiency}
\newglossaryentry{s87}{type=symbols,name=$q$,description= non-negative constant}







